On Constraints in First-Order Optimization: A View from Non-Smooth Dynamical Systems

We introduce a class of first-order methods for smooth constrained optimization that are based on an analogy to non-smooth dynamical systems. Two distinctive features of our approach are that (i) projections or optimizations over the entire feasible set are avoided, in stark contrast to projected gradient methods or the Frank-Wolfe method, and (ii) iterates are allowed to become infeasible, which differs from active set or feasible direction methods, where the descent motion stops as soon as a new constraint is encountered. The resulting algorithmic procedure is simple to implement even when constraints are nonlinear, and is suitable for large-scale constrained optimization problems in which the feasible set fails to have a simple structure. The key underlying idea is that constraints are expressed in terms of velocities instead of positions, which has the algorithmic consequence that optimizations over feasible sets at each iteration are replaced with optimizations over local, sparse convex approximations. In particular, this means that at each iteration only constraints that are violated are taken into account. The result is a simplified suite of algorithms and an expanded range of possible applications in machine learning.

==> virtWork.tex <==
\section{The principle of virtual work}
\subsection{The static equilibrium}
We consider the following optimization problem 
\begin{equation}
\min_{x\in \mathbb{R}^{n}} f(x),\quad \text{s.t.}\quad g(x)\geq 0, h(x)=0, \label{eq:fundProb}
\end{equation}
where the continuously differentiable function $f:\mathbb{R}^{n}\rightarrow \mathbb{R}$ defines the objective function and the continuously differentiable functions $g:\mathbb{R}^{n} \rightarrow \mathbb{R}^{n_\text{g}}$ and $h:\mathbb{R}^{n} \rightarrow \mathbb{R}^{n_\text{h}}$, define the constraints. The variables $n$, $n_\text{g}$, and $n_\text{h}$ are integers and $\mathbb{R}$ denotes the real numbers. We denote the set of all $x\in \mathbb{R}^n$ that satisfy the constraints $g(x)\geq 0$ and $h(x)=0$ by $C$, which we assume to be non-empty and bounded.\footnote{The assumption of $C$ being bounded could be replaced by the assumption that the function $f$ is such that $f(x) \rightarrow \infty$ for $|x|\rightarrow \infty$.} The set $C$ is therefore compact, which implies that the minimum in \eqref{eq:fundProb} is attained. We make the following additional assumption on the set $C$.
\begin{assumption} (Mangasarian-Fromovitz constraint qualification)\label{Ass:Fund}
For any $x\in C$ the rows of $\left.\partial h/\partial x\right|_{x}$ are linearly independent. Moreover, there exists a vector $w\in \mathbb{R}^n$ such that $\left.\partial h/\partial x\right|_{x} w=0$, $\left.\partial g_{I(x)}/\partial x\right|_{x} w > 0$, where $I(x)$ denotes the active inequality constraints, i.e. $I(x):=\{i\in \mathbb{Z}~|~g_i(x)=0\}$.
\end{assumption}
According to \citet[p.~209, p.~221, p.~226]{Rockafellar} this implies that the set $C$ is regular (in the sense of Clarke) and geometrically derivable.
%\textcolor{red}{Maybe even Abadie constraint qualification (weaker) is possible.}

Let $x^*$ denote a local minimum of \eqref{eq:fundProb}. This means that $f(\bar{x})\geq f(x^*)$ for any $\bar{x}$ in an open neighborhood of $x^*$ that satisfies the constraints, or equivalently
\begin{equation}
-\delta f:=-\left.\frac{\partial f}{\partial x}\right|_{x^*} \delta x \leq 0, \quad \forall \delta x \in T_{C}(x^*), \label{eq:statCond}
\end{equation}
where $T_{C}(x^*)$ denotes the tangent cone to the constraint set $C$. In other words, variations of the function $f$ (denoted $\delta f$) are positive for all variations $\delta x$ that are in accordance with the constraints. These variations will be called admissible, i.e. $\delta x \in T_C(x^*)$. A variation $\delta x$ represents an infinitesimal change in $x$ and, due to the fact that $C$ is geometrically derivable by Assumption~\ref{Ass:Fund}, can be represented as the right-sided derivative of a function,
\begin{equation}
\delta x=\lim_{t\downarrow 0} \frac{\xi(t)-\xi(0)}{t}, \quad \xi(0)=x^*,
\end{equation} 
where $\xi:[0,\epsilon] \rightarrow \mathbb{R}^{n}$ is any function that has a right-sided derivative at $0$, and $\epsilon>0$ is a small real number. Admissible variations are obtained if the functions $\xi$ are restricted to $\xi:[0,\epsilon]\rightarrow C$. %We use the symbol $\delta$ to emphasize that the variation is a \emph{virtual} change, that is, $\delta f$ for example refers to the value of $f$ if we \emph{were} to evaluate it at an arbitrarily close point $x^*+\delta x$ compared to $f(x^*)$. In contrast, the symbol $\text{d}$ will be reserved for the differential with respect to time of a trajectory and should therefore be distinguished from $\delta$. In \eqref{eq:statCond} only variations are considered that are in accordance with the constraints. 
As a result of the chain rule, the admissible variations are therefore given by
\begin{equation*}
T_{C}(x^*):=\{ \delta x \in \mathbb{R}^n~|~ \left.\frac{\partial h}{\partial x}\right|_{x^*} \delta x = 0, \left.\frac{\partial g_{I(x^*)}}{\partial x}\right|_{x^*} \delta x \geq 0\},
\end{equation*}
where the index set $I(x^*)$ denotes all the active constraints, c.f. Assumption~\ref{Ass:Fund}.

The stationarity condition \eqref{eq:statCond} can also be expressed in the following equivalent way: 
\begin{equation}
-\left.\frac{\partial f}{\partial x}\right|_{x^*}\T + R = 0, \quad \text{for~some}~-R\in N_C(x^*), \label{eq:KKT}
\end{equation}
where the normal cone $N_C(x^*)$ denotes the set of all vectors that satisfy
\begin{equation}
N_C(x^*):=\{\lambda \in \mathbb{R}^n~|~\lambda\T \delta x \leq 0, \forall \delta x\in T_C(x^*)\}.
\end{equation}
Equivalently, the condition \eqref{eq:KKT} can be expressed using a variational equality,
\begin{equation}
(-\left.\frac{\partial f}{\partial x}\right|_{x^*} + R\T)\delta x= 0, \quad \forall \delta x\in \mathbb{R}^n, \quad \text{for~some}~-R\in N_C(x^*). \label{eq:varForm}
\end{equation}
Compared to \eqref{eq:statCond}, the variations in \eqref{eq:varForm} are unconstrained. Thus, the procedure for obtaining \eqref{eq:varForm} amounts to replacing the geometric boundary conditions ($\delta x \in T_C(x^*)$) via the Lagrange multipliers $R$, which are normal to $T_C(x^*)$. The conditions \eqref{eq:statCond}, \eqref{eq:KKT}, and \eqref{eq:varForm} are therefore all equivalent, \eqref{eq:KKT} essentially being the Karush-Kuhn-Tucker conditions of optimality.

We now proceed to give an mechanical interpretation for the conditions \eqref{eq:statCond}, \eqref{eq:KKT}, and \eqref{eq:varForm} by considering a point mass on which the external force $F:=-\partial f/\partial x\T$ acts. 
%
%In order to simplify the presentation we assume
%\begin{assumption}\label{Ass:Regular}
%The set $C$ is regular in the sense of Clarke, see \cite[p.~199]{Rockafellar}. This means that for any $x\in C$ and any converging sequence $\lambda_k \in N_C(x_k)$, where $x_k\in C$, $x_k\rightarrow x$, it holds that $\lim_{k\rightarrow \infty} \lambda_k \in N_C(x)$.
%\end{assumption}
%The assumption excludes so-called inward facing corners, as shown in Fig.~\ref{Fig:Inward}, and will be discussed further below.
%
%Alternatively, the constraints can be included in the objective function. To that extent we introduce the extended real numbers $\bar{\mathbb{R}}=\{-\infty,\infty\} \cup \mathbb{R}$ and define the two indicator functions $\psi_{0}:\mathbb{R}^{n_\text{h}}\rightarrow \bar{\mathbb{R}}$ and $\psi_{\geq 0}:\mathbb{R}^{n_\text{g}}\rightarrow \bar{\mathbb{R}}$ in the following way
%\begin{equation*}
%\psi_{0}(x)=\begin{cases} \infty &x \neq 0,\\
%0 &x=0,\end{cases} \quad \psi_{\geq 0}(x)=\begin{cases} \infty &x\geq 0,\\ 0 &x=0.\end{cases}
%\end{equation*}
%As a consequence the optimization problem \eqref{eq:fundProb} can be rewritten as 
%\begin{equation}
%\min_{x\in \mathbb{R}^{n}} f(x) + \psi_0(h(x)) + \psi_{\geq 0}(g(x)),
%\end{equation}
%which concludes that the optimum $x^*$ satisfies
%
%If certain regularity conditions are met, it can be shown that \eqref{eq:statCond} is equivalent to
%\begin{equation}
%\left(-\left.\frac{\partial f}{\partial x}\right|_{x^*} + \lambda_\text{h}\T \left.\frac{\partial h}{\partial x}\right|_{x^*} + \lambda_\text{g}\T \left.\frac{\partial g}{\partial x}\right|_{x^*} \right) \delta x \leq 0, \quad \forall \delta x \in \mathbb{R}^n, \label{eq:varForm}
%\end{equation}
%for a $-\lambda_\text{h}\in \partial \psi_{0}(h(x^*))$ and a $-\lambda_\text{g} \in \partial \psi_{\geq 0}(g(x^*))$. The subgradients of the indicator functions $\psi_0$ and $\psi_{\geq 0}$ are denoted by $\partial \psi_0$ and $\partial \psi_{\geq 0}$, respectively, whereas $\psi_0$ and $\psi_{\geq 0}$ are extended real-valued functions defined by
%\begin{equation*}
%\psi_{0}(x)=\begin{cases} \infty &x \neq 0,\\
%0 &x=0,\end{cases} \quad \psi_{\geq 0}(x)=\begin{cases} \infty &x\geq 0,\\ 0 &x=0.\end{cases}
%\end{equation*}
%Compared to \eqref{eq:statCond}, the variations in \eqref{eq:varForm} are unconstrained. In addition, since for any $\delta x$, $-\delta x$ is likewise an admissible variation, the inequality in \eqref{eq:varForm} reduces to an equality, which implies that \eqref{eq:varForm} is equivalent to the well-known Karush-Kuhn-Tucker conditions of \eqref{eq:fundProb}
%\begin{equation}
%-\left.\frac{\partial f}{\partial x}\right|_{x^*}\T + \left.\frac{\partial h}{\partial x}\right|_{x^*}\T \lambda_\text{h} + \left.\frac{\partial g}{\partial x}\right|_{x^*}\T \lambda_\text{g} = 0. \label{eq:KKT}
%\end{equation}
We further assume that the point mass' position is described by $x$, and that it is constrained to the set $C$. For a given $\bar{x}$ we investigate if the point mass is in a static equilibrium, i.e. does not move under the laws of physics. In order to do so, we construct a free body diagram, where we replace the geometric constraint $x\in C$ with constraint forces. The graphical procedure is illustrated in Fig.~\ref{Fig:ill} on three simple examples. Mathematically, this graphical cutting principle amounts to replacing the geometric constraints by constraint forces $-R\in N_{C}(\bar{x})$. The principle of virtual work, which is sometimes regarded as the fundamental postulate of classical mechanics, states that
\begin{postulate}
The point mass is in static equilibrium if and only if the virtual work vanishes for any virtual displacement $\delta x$. The virtual work is defined as $(F+R)\T \delta x$, where $F$ is the sum of all external forces and $R$ is the sum of all constraint forces.
\end{postulate}
Thus, with our choice $F:=-\partial f/\partial x\T$ we can relate the stationarity conditions of \eqref{eq:fundProb}, given by the Karush-Kuhn-Tucker conditions \eqref{eq:varForm} to the static equilibrium of a point mass, as characterized by the principle of virtual work. By definition, constraint forces satisfy $-R\T \delta x \leq 0$ for all $\delta x \in T_C(\bar{x})$, or in the language of classical mechanics: constraint forces are such that the their contribution to the virtual work is non-negative.\footnote{In most classical textbooks only equality constraints are considered. In that case constraint forces exert no virtual work.} This leads to the principle of d'Alembert-Lagrange, which represents the basis for most classical mechanics
\begin{corollary}\label{Cor:DAlembertLagrange}
If the point mass located at $x^*\in C$ is in static equilibrium, the virtual work of the external forces satisfies $F\T \delta x \leq 0$ for all admissible variations $\delta x$, i.e. $\delta x\in T_C(x^*)$.
\end{corollary}
Thus, the principle of d'Alembert-Lagrange encodes \eqref{eq:statCond}. Whereas in optimization, one typically starts with the stationarity condition \eqref{eq:statCond} and then derives the Karush-Kuhn-Tucker conditions \eqref{eq:KKT}, the workflow in mechanics is often in the reverse direction. Starting from a free-body diagram, one would like to eliminate as many constraint forces as possible by an appropriate choice of coordinates, which amounts to applying the principle of D'Alembert-Lagrange. As the physicist C. Lanczos beautifully describes in \cite{bookLanczos}: ``This form (the principle of virtual work) isolates the particle and replaces all constraints by forces. The inconvenience of this procedure is obvious if we think of such a simple problem as the equilibrium of a lever. The lever is composed of an infinity of particles and an infinity of inner forces acting between them. The analytical treatment (principle of D'Alembert-Lagrange) can dispense with all the forces and take only the external force, i.e. in this case the force of gravity, into account. This is accomplished by performing only such virtual displacements (variations) that are in harmony with the given constraints. In case of the lever, for example, we let the lever rotate around its fulcrum, as a rigid body, thus preserving the mutual distances of any two particles. By this procedure the inner forces, which produce the constraints need not be considered."

It is interesting to note what happens if Assumption~\ref{Ass:Fund} is omitted, more precisely, if the set $C$ fails to be regular in the sense of Clarke. In that case the definition of the set $N_C(x^*)$ should be extended to be the polar of the regular tangent cone, c.f. \cite[p.~217]{Rockafellar}. In the context of optimization this not too much of an issue: Even though \eqref{eq:varForm} and \eqref{eq:statCond} are no longer equivalent, \eqref{eq:statCond} still implies \eqref{eq:varForm} (the set $N_C(x^*)$ has been enlarged), and therefore \eqref{eq:varForm} is still a necessary condition for local optimality. In mechanics the situation is more troubling. The lack of equivalence between \eqref{eq:statCond} and \eqref{eq:varForm} implies that the principle of d'Alembert-Lagrange, at least as stated in Corollary~\ref{Cor:DAlembertLagrange}, is no longer a consequence of the principle of virtual work and therefore ceases to hold, \cite{Panagiotopoulous}. However, the fundamental analogy between the principle of virtual work and the Karush-Kuhn-Tucker conditions \eqref{eq:varForm} still applies. 

\subsection{The dynamic equilibrium}
Until now, we provided an analogy between the stationarity conditions of a constrained optimization problem and the static equilibrium of a mechanical system. However, the important insight from classical mechanics (essentially due to d'Alembert) is that the principle of virtual work, Postulate~\ref{Pos:VirtWork}, and the principle of D'Alembert-Lagrange, Corollary~\ref{Cor:DAlembertLagrange}, naturally extend to the \emph{dynamic} equilibrium of a mechanical system. It suffices to add the ``forces of inertia", which for mechanical systems typically amounts to $-m \ddot{x}$, to the external forces. As we point out in the following, these ideas naturally extend to the design of optimization algorithms.

In order to fix the ideas we start by considering gradient flow. We will then proceed to accelerated gradient flow. It is clear that the fundamental procedure applies to almost any continuous-time and discrete-time optimization algorithm. Gradient flow for unconstrained minimization is given by
\begin{equation}
\dot{x}(t)=-\left.\frac{\partial f}{\partial x}\right|_{x(t)}\T, \quad \text{or~equivalently,} \quad \left(-\dot{x}(t)\T - \left.\frac{\partial f}{\partial x}\right|_{x(t)} \right) \delta x(t) \leq 0, \quad \forall \delta x(t) \in \mathbb{R}^n,\label{eq:gradFlow}
\end{equation}
and is known to converge to a local minimum of $f$ from a large number of initial conditions. By analogy to the principle of d'Alembert-Lagrange we therefore require
\begin{equation}
\left(-\dot{x}(t)\T-\left.\frac{\partial f}{\partial x}\right|_{x(t)}\right) \delta x(t) \leq 0 \quad \forall \delta x(t) \in T_{C}(x(t)), \quad \forall t \in [0,\infty)~\text{a.e.} \label{eq:cond1}
\end{equation}
to obtain a constrained optimization algorithm.
Compared to the stationarity condition \eqref{eq:statCond}, which prescribes the gradient at a single point $x^*\in C$, it is important to realize that \eqref{eq:cond1} represents a condition on the whole trajectory $x: [0,\infty) \rightarrow \mathbb{R}^n$. Moreover, in contrast to \eqref{eq:gradFlow}, the velocity $\dot{x}$ is allowed to ``jump", for example when $x(t)$ approaches the boundary of the constraint $C$, since \eqref{eq:cond1} applies only for almost all $t\in [0,\infty)$. As pointed out in \citet[p.~1]{Filippov}, for example, this requires a generalization of the concept of a solution, which typically needs to take the underlying purpose (or physical meaning) of the given problem into account. We will therefore restrict ourselves to the following trajectories.
\begin{assumption}\label{Ass:Sol}
The trajectory $x:[0,\infty) \rightarrow \mathbb{R}^n$ is a solution to \eqref{eq:cond1} if it satisfies \eqref{eq:cond1}, is absolutely continuous and has a derivative (almost everywhere) that is of locally bounded variation.
\end{assumption}
This means that on any compact time interval, $\dot{x}$ is continuous except on a countable set of points, at which the left and right one-sided limits of $\dot{x}$, denoted by $\dot{x}^-(t)$ and $\dot{x}^+(t)$, respectively, still exist. We will show in the remainder that this solution concept is indeed reasonable and useful in the context of optimization.

In addition, we note that the constraint $x(t)\in C$ is implicit in the requirement $\delta x(t)\in T_C(x(t))$, and that the variations $\delta x(t)$ and $\delta x(t')$ for $t\neq t'$ are assumed to be unrelated.

The condition \eqref{eq:cond1} is equivalent to 
\begin{equation}
\dot{x}(t)=-\frac{1}{L} \left.\frac{\partial f}{\partial x}\right|_{x(t)}\T + R(t), \quad -R(t)\in N_C(x(t)), \quad \forall t\in [0,\infty)~\text{a.e.}, \label{eq:cond2}
\end{equation}
where the requirement $x(t)\in C$ is again implicit in $-R(t)\in N_C(x(t))$. The right-hand side of \eqref{eq:cond2} is set valued, which makes it explicit that \eqref{eq:cond2} and \eqref{eq:cond1} represent a differential inclusion. The assumption of the trajectory $x$ being absolutely continuous amounts to the classical solution concept introduced in \cite{Filipov}. 

Summarizing, by analogy to the principle of D'Alembert-Lagrange we obtained the differential inclusion \eqref{eq:cond2}, which generalizes \eqref{eq:gradFlow} to constrained optimization. The constraints are formulated on position level, and as is shown in App.~\ref{App:CTAnalogue}, \eqref{eq:finalGDpos} can be regarded as the continuous-time analogue of projected gradient descent.

Next we exploit the structure of the set $C$ to further simplify \eqref{eq:cond2}, ultimately leading to a discrete-time algorithm that optimizes \eqref{eq:fundProb}. The following lemma from \cite[p.~202]{Rockafellar}, which can be interpreted as a coordinate transformation, represents a first step:
\begin{lemma}\label{Lemma:LICQ}
As a consequence of Assumption~\ref{Ass:Fund}, $N_C(x)$ can be expressed as
\begin{equation}
N_C(x):=\{-\frac{\partial h}{\partial x}\T \lambda_\text{h} - \frac{\partial g}{\partial x} \T \lambda_\text{g}~|~-\lambda_\text{h} \in N_{\{0\}}(h(x)), -\lambda_\text{g} \in N_{\mathbb{R}_{\geq 0}}(g(x))\}. \label{eq:NCsimplification}
\end{equation}
\end{lemma}
The constants $\lambda_\text{h}$ and $\lambda_\text{g}$ are commonly referred to as Lagrange multipliers, and represent the magnitudes of the constraint forces in a mechanical analogy. The set-valued functions $N_{\{0\}}(h(x))$ and $N_{\mathbb{R}_{\geq 0}}(g(x))$ are illustrated in Fig.~\ref{Fig:NConeInclusion}, which shows that the conditions $-\lambda_\text{h} \in N_{\{0\}}(h(x))$ and $-\lambda_\text{g}\in N_{\mathbb{R}_{\geq 0}}(g(x))$ can be expressed as 
\begin{equation}
\lambda_{\text{h}i}\in \mathbb{R},~~ h_i(x)=0, \qquad \lambda_{\text{g}j}\geq 0,~~ g_j(x)\geq 0,~~ \lambda_{\text{g}j} g_j(x)=0, \label{eq:posLevel}
\end{equation}
for all $i=1,\dots,n_\text{h}$ and all $j=1,\dots,n_\text{g}$. As a result, \eqref{eq:cond2} can be reformulated as
\begin{multline}
\dot{x}(t)=-\left.\frac{\partial f}{\partial x}\right|_{x(t)}\T + \left.\frac{\partial h}{\partial x}\right|_{x(t)}\T \lambda_{\text{h}}(t) + \left.\frac{\partial g}{\partial x}\right|_{x(t)}\T \lambda_{\text{g}}(t), \\
-\lambda_\text{h}(t)\in N_{\{0\}}(h(x(t)), \quad -\lambda_\text{g}(t)\in N_{\mathbb{R}_{\geq 0}}(g(x(t)), \quad \forall t\in [0,\infty)~\text{a.e.}\label{eq:finalGDpos}
\end{multline}
%This represents a condition on the whole trajectory $x$, satisfying Ass.~\ref{Ass:Sol}. 
Evaluating the right-hand side of \eqref{eq:finalGDpos} for a specific $x(t)$ at a specific time instant $t$ is not straightforward, since implicit constraints on the variables $\lambda_\text{h}(t)$ and $\lambda_\text{g}(t)$ need to be taken into account. In particular, $\lambda_\text{h}(t)$ and $\lambda_\text{g}(t)$ must be chosen exactly in such a way that $x(\bar{t})$ remains in $C$ for any sufficiently small time instant $\bar{t}>t$. In other words, the constraint $x(t)\in C$ for all $t\in [0,\infty)$ induces constraints on $\dot{x}$. As will be shown in the next section, an explicit description of the motion described by \eqref{eq:finalGDpos}, i.e. $x(\bar{t})$ given $x(t)$ for $\bar{t}>t$ or $\bar{t}<t$, can be obtained by reformulating the constraint $x(t)\in C$ in terms of the induced constraint on velocity level.

%We conclude the section by summarizing the properties of \eqref{eq:finalGDpos}, a proof of which is deferred to the next section.
%\begin{proposition}
%The dynamics \eqref{eq:finalGDpos} represent a continuous-time optimization algorithm for \eqref{eq:fundProb}. The function $f$ necessarily decreases along trajectories. For strongly convex functions the convergence rate is given by 
%\begin{equation}
%|x(t)-x^*|\leq |x(0)-x^*| e^{-\mu t/L}, \quad \forall t\in [0,\infty).
%\end{equation}
%where $L>0$ and $\mu>0$ refer to the smoothness and strong convexity constant of $f$.
%\end{proposition}
%\begin{proof}
%The fact that $f$ decreases along trajectories is immediate. We multiply \eqref{eq:finalGDpos} with $\dot{x}(t)$,
%\begin{align}
%|\dot{x}(t)|^2 = -\frac{\diff}{\diff t}(f(x(t)) + \dot{x}(t)\T \left. \frac{\partial h}{\partial x}\right|_{x(t)}\T \lambda_\text{h}(t) + \dot{x}(t)\T \left.\frac{\partial g}{\partial x}\right|_{x(t)}\T \lambda_\text{g}(t)
%\end{align}
%and note that due to the fact that $x(t)\in C$, $\partial h/\partial x|_{x(t)} \dot{x}(t)=0$. Moreover, since $\dot{x}(t)\T \partial g_I/\partial x|_{x(t)}$
%\end{proof}

\section{Reformulating the constraints on the velocity level}

We start by defining the rate of change of the constraints
\begin{equation*}
\gamma_{\text{h}}(\dot{x}(t),x(t)):=\left.\frac{\partial h}{\partial x}\right|_{x(t)} \dot{x}(t), \quad \gamma_{\text{g}}(\dot{x}(t),x(t)):=\left.\frac{\partial g}{\partial x}\right|_{x(t)} \dot{x}(t),
\end{equation*} 
which are, due to Ass.~\ref{Ass:Sol}, of locally bounded variation. This means that both $\gamma_\text{h}$ and $\gamma_\text{g}$ are continuous except for countably many points, at which their left and right limits, denoted by $\gamma_\text{h}^-$ and $\gamma_\text{g}^-$, respectively $\gamma_\text{h}^+$ and $\gamma_\text{g}^+$ still exist. We consider the equality constraint first. Due to the absolute continuity of $x(t)$, the condition $h(x(t))=0$ is equivalent to $\gamma_\text{h}^+(x(t),\dot{x}(t))=0$ for all $t\in [0,\infty)$, $h(x(0))=0$, and we obtain 
\begin{equation}
h(x(0))=0,~-\lambda_\text{h}^+(t)\in N_{\{0\}}(\gamma_{\text{h}}^+(\dot{x}(t),x(t))) \quad \Leftrightarrow \quad -\lambda_{\text{h}}(t) \in N_{\{0\}}(h(x(t))),  \label{eq:velLevel1}
\end{equation}
where the left condition applies for all $t\in [0,\infty)$ and the right for all $t\in [0,\infty)$ (a.e.), and $\lambda_\text{h}(t)$ is assumed to be of locally bounded variation (in accordance with $\dot{x}$).
Compared to the condition in \eqref{eq:posLevel}, it is important to emphasize that the equivalence in \eqref{eq:velLevel1} applies to whole trajectories. An similar equivalence can be expressed for the backwards motion, which amounts to replacing $\lambda_\text{h}^+$ and $\gamma_\text{h}^+$ with $\lambda_\text{h}^-$ and $\gamma_\text{h}^-$, and $h(x(0))=0$ with $\lim_{t\rightarrow \infty} h(x(t))=0$ in \eqref{eq:velLevel1}.

The inequality constraints are more delicate. We start by assuming that the $i$'th constraint is closed at time $\bar{t}$, i.e. $g_i(x(\bar{t}))=0$, $\lambda_{\text{g}i}(\bar{t})\geq 0$. Two scenarios are possible: 1) The constraint $g_i(x(t))$ opens, i.e. $g_i(x(t))>0$ for any sufficiently small $t>\bar{t}$, which is equivalent to $\gamma_{\text{g}i}^+(\dot{x}(\bar{t}),x(\bar{t}))>0$ or 2) the constraint $g_i(x(t))$ remains closed, i.e. $g_i(x(t))=0$ for any sufficiently small $t>\bar{t}$, which is equivalent to $\gamma_{\text{g}i}^+(\dot{x}(\bar{t}),x(\bar{t}))=0$. In the former case the constraint force $\lambda_{\text{g}i}(t)$ vanishes for any sufficiently small $t>\bar{t}$, i.e. $\lambda_{\text{g}i}^+(\bar{t})=0$. In the latter case, we have $\lambda_{\text{g}i}^+(\bar{t})\geq 0$. If the constraint $i$ is open at time $\bar{t}$, i.e. $g_i(x(\bar{t}))>0$, it follows that $\lambda_{\text{g}i}(\bar{t})=\lambda_{\text{g}i}^+(\bar{t})=0$. This indicates that the relations \eqref{eq:posLevel} can be reformulated as
\begin{equation}
-\lambda_{\text{g}j}(t) \in N_{\mathbb{R}_{\geq 0}}(g_j(x(t)) \quad \Leftrightarrow \quad -\lambda_{\text{g}j}^+(t) \in \begin{cases} 0 &g_j(x(t))>0\\
0 &g_j(x(t))=0, \gamma_{\text{g}j}(\dot{x}(t),x(t))^+>0\\
[-\infty,0] &g_j(x(t))=0, \gamma_{\text{g}j}(\dot{x}(t),x(t))^+=0, \end{cases}\label{eq:velLevel2}
\end{equation}
for $j=1,\dots,n_{\text{g}}$, where again the first conditions applies for all $t\in [0,\infty)$ (a.e.), and the second for all $t\in [0,\infty)$, whereby $\lambda_{\text{g}j}$ is assumed to be of locally bounded variation. The above argument shows the first implication of \eqref{eq:velLevel2}, the reverse direction is immediate. As in \eqref{eq:velLevel1}, \eqref{eq:velLevel2} is formulated for the forward motion. An equivalent formulation in terms of the backwards motion is possible.

In view of \eqref{eq:velLevel1} and \eqref{eq:velLevel2} we can therefore express \eqref{eq:finalGDpos} in the following way
\begin{multline}
\dot{x}=-\left.\frac{\partial f}{\partial x}\right|_{x}\T + \left.\frac{\partial h}{\partial x}\right|_{x}\T \lambda_{\text{h}} + \left.\frac{\partial g}{\partial x}\right|_{x}\T \lambda_{\text{g}}, \quad
-\lambda_\text{h}^+\in N_{\{0\}}(\gamma_\text{h}^+(\dot{x},x)), \\
-\lambda_{\text{g}I^\text{c}(x)}^+=0,\quad -\lambda_{\text{g}I(x)}^+\in N_{\mathbb{R}_{\geq 0}}(\gamma_{\text{g}I(x)}^+(\dot{x},x)), \quad \forall t\in [0,\infty)~\text{a.e.},\label{eq:finalGDvel}
\end{multline}
where the index set $I^{\text{c}}(x)$ denotes the set of all open constraints, that is, $I^{\text{c}}(x):=\{i\in \mathbb{Z}~|~g_i(x)>0\}$, and where the dependence on time has been omitted. In contrast to \eqref{eq:finalGDpos}, \eqref{eq:finalGDvel} explicitly describes the forward evolution of the trajectory $x(t)$: By assumption $\dot{x}$ is of locally bounded variation and therefore there are only countably many points where $\dot{x}$ can be discontinuous. In case $\dot{x}(t)$ is continuous in an open interval containing $t$, the right-sided limits in \eqref{eq:finalGDvel} become superfluous, and, as shown below, $\dot{x}(t)$ is fully determined through the implicit relations in \eqref{eq:finalGDvel}. In case $\dot{x}(t)$ happens to be discontinuous at time $t$, its right-sided limit is still well-defined and, according to \eqref{eq:finalGDvel}, determined by
\begin{equation*}
\dot{x}^+(t)=-\left.\frac{\partial f}{\partial x}\right|_{x(t)}\T + \left.\frac{\partial h}{\partial x}\right|_{x(t)}\T \lambda_{\text{h}}^+(t) + \left.\frac{\partial g}{\partial x}\right|_{x(t)}\T \lambda_{\text{g}}^+(t),
\end{equation*}
where the multipliers $\lambda_\text{g}^+(t)$ and $\lambda_\text{h}^+(t)$ satisfy the conditions in \eqref{eq:finalGDvel}. The right-limit $\dot{x}^+(t)$ then prescribes the evolution of $x(\tau)$ for $\tau>t$. In both cases we end up with the same algebraic conditions that determine $\dot{x}(t)$ or $\dot{x}^+(t)$, respectively. From now on, we will therefore simplify notation and omit the right-sided limit $^+$. For a fixed time $t$, \eqref{eq:finalGDvel} can be rewritten more compactly as
\begin{align}
\dot{x}+\left.\frac{\partial f}{\partial x}\right|_{x}\T = W \lambda, \quad -\lambda\in N_{D}(W\T \dot{x}), \quad W:=\left(\left.\frac{\partial h}{\partial x}\right|_{x}\T, \left.\frac{\partial g_{I(x)}}{\partial x}\right|_{x}\T\right), \label{eq:tmp1}
\end{align}
where $D:=\{0\}^{n_\text{h}} \times \mathbb{R}_{\geq 0}^{|I(x)|}$, with $|I(x)|$ the cardinality of $I(x)$, and where the dependence on time has been omitted. 

In order to interpret \eqref{eq:tmp1} we introduce the set $\dot{C}(x)\subset\mathbb{R}^n$, as the induced constraint on velocity level, i.e.
\begin{equation*}
\dot{C}(x):=\{\dot{x}\in \mathbb{R}^n~|~W\T \dot{x} \in D\}=\{\dot{x} \in \mathbb{R}^n~|~\left.\frac{\partial h}{\partial x}\right|_{x} \dot{x}=0,~\left.\frac{\partial g_{I(x)}}{\partial x}\right|_{x} \dot{x} \geq 0\},
\end{equation*}
where the last equality follows from the definition of the matrix $W$.
As a result of Assumption~\ref{Ass:Fund}, we can apply Lemma~\ref{Lemma:LICQ} (with $C$ replaced by $\dot{C}$), which characterizes the set of normal vectors
\begin{equation*}
N_{\dot{C}(x)}(\dot{x}) = \{-W \lambda ~|~-\lambda \in N_D(W\T \dot{x})\}.
\end{equation*}
We therefore conclude that \eqref{eq:tmp1} can be rewritten as
\begin{equation}
\left( \dot{x}(t)\T+\left.\frac{\partial f}{\partial x}\right|_{x(t)}-R(t)\T\right) \delta v(t)=0, \quad \forall \delta v(t)\in \mathbb{R}^n, \quad -R(t)\in N_{\dot{C}(x(t))}(\dot{x}(t)), \label{eq:virtPower}
\end{equation}
or equivalently as
\begin{equation}
\left( -\dot{x}(t)\T-\left.\frac{\partial f}{\partial x}\right|_{x(t)}\T \right) \delta v(t)\leq 0, \quad \forall \delta v(t)\in T_{\dot{C}(x(t))}(\dot{x}(t)). \label{eq:principleJourdain}
\end{equation}
In mechanics the former is known as the principle of virtual power. In other words, a mechanical system is in dynamic equilibrium if and only the virtual power, the product between forces and virtual velocities, vanishes for any virtual velocity. The latter is known as the principle of Jourdain. Compared to the principle of D'Alembert-Lagrange it can account for constraints on velocity level, and is therefore more general. In addition, since gradient flow is a first-order differential equation, \eqref{eq:principleJourdain} can be interpreted as stationarity condition of the following convex optimization problem
\begin{equation}
\min_{\dot{x}(t)\in \mathbb{R}^n} \frac{1}{2} \Big| \dot{x}(t) + \left.\frac{\partial f}{\partial x}\right|_{x(t)}\T \Big|^2 \quad \text{s.t.} \quad \dot{x}(t)\in \dot{C}(x(t)). \label{eq:principleGauss}
\end{equation}
It is important to note that the set $\dot{C}(x)$ is convex, by construction. The optimization problem \eqref{eq:principleGauss} provides a clear interpretation of the dynamics given by \eqref{eq:cond1} (or alternatively \eqref{eq:tmp1}): for a given $x(t)$ the velocity $\dot{x}(t)$ at time $t$ (or $\dot{x}^+(t)$ if $\dot{x}(t)$ happens to be discontinuous at $t$) is precisely the velocity that is closest to standard gradient flow \eqref{eq:gradFlow}, subject to the constraint $\dot{x}(t) \in \dot{C}(x(t))$. Since the constraint $\dot{C}(x(t))$ is by virtue of Ass.~\ref{Ass:Fund} non-empty, closed, and convex for all $x(t)$ the velocity $\dot{x}(t)$ (or $\dot{x}^+(t)$) is well-defined and unique for each $x(t)\in C$. 

There is yet another way to express \eqref{eq:tmp1}. Taking advantage of the fact that $D$ is a convex cone, the normal cone inclusion $-\lambda \in N_D(W\T \dot{x})$ is equivalent to $W\T \dot{x} \in N_{D^*}(-\lambda)$, where $D^*$ is the polar cone, i.e. $D^*=\mathbb{R}^{n_\text{h}} \times \mathbb{R}_{\leq 0}^{|I(x)|}$. Eliminating $\dot{x}$ in \eqref{eq:tmp1} then yields
\begin{equation}
W\T W \lambda - W\T \left.\frac{\partial f}{\partial x}\right|_{x}\T \in N_{D^*}(-\lambda) \quad \Leftrightarrow \quad \min_{\lambda} \frac{1}{2} \Big|W \lambda - \left.\frac{\partial f}{\partial x}\right|_{x}\T\Big|^2, ~~ \text{s.t.} ~~ -\lambda \in D^*, \label{eq:dualProb}
\end{equation}
which corresponds to the dual problem of \eqref{eq:principleGauss}. According to \eqref{eq:tmp1}, the cost function in \eqref{eq:dualProb} can be interpreted as $|\dot{x}|^2$. This yields the following interpretation: At each point in time the constraint forces $\lambda \in -D^*$ are chosen to minimize the velocity. The velocity characterizes the distance to an equilibrium, which corresponds to a stationary point of \eqref{eq:fundProb}.


We can therefore summarize our findings:
\begin{proposition}\label{Prop:ConvGD}
Under Assumption~\ref{Ass:Fund} and Assumption~\ref{Ass:Sol}, the constrained gradient flow as given by \eqref{eq:cond1}, \eqref{eq:cond2}, \eqref{eq:finalGDpos}, \eqref{eq:finalGDvel}, \eqref{eq:tmp1}, \eqref{eq:virtPower}, \eqref{eq:principleJourdain}, \eqref{eq:principleGauss}, or \eqref{eq:dualProb} has well-defined and unique solutions in forward time. The objective function $f$ necessarily decreases along trajectories and $x(t)$ converges to a stationary point of \eqref{eq:fundProb}. In case $f$ is strongly convex and smooth, and the set $C$ is convex, the trajectories converge with rate
\begin{equation*}
|f(x(t))-f^*|\leq |f(x(0))-f^*| e^{-\mu t/L},
\end{equation*}
where $f^*$ denotes the value of the minimum in \eqref{eq:fundProb}.
\end{proposition}
\begin{proof}
We use the formulation \eqref{eq:tmp1}, which we multiply by $\dot{x}(t)$. This yields
\begin{equation*}
|\dot{x}(t)|^2 = -\frac{\diff}{\diff t} f(x(t)) + \dot{x}(t)\T W(t) \lambda(t).
\end{equation*}
Due to the fact that $\dot{x}(t)\T W(t) \lambda(t)=0$ for all times $t$ we obtain
\begin{equation}
\frac{\diff}{\diff t} f(x(t)) = -|\dot{x}(t)|^2\leq 0, \label{eq:last}
\end{equation}
which proves that $f(x(t))$ strictly decreases. Thus $f(x(t))$ converges for $t\rightarrow \infty$, and we have $\lim_{t\rightarrow \infty} \dot{x}^+(t)=0$, which implies, according to \eqref{eq:cond2}, that $\lim_{t\rightarrow \infty} x(t)$ satisfies the Karush-Kuhn-Tucker conditions \eqref{eq:KKT}. 

We now proceed to the case where $f$ is strongly convex and $C$ is convex. We can rewrite the equality \eqref{eq:last} as
\begin{equation}
\frac{\diff}{\diff t} f(x(t)) = -\Big|\left.\frac{\partial f}{\partial x}\right|_{x(t)} - R(t)\Big|^2, \label{eq:tmpproof1}
\end{equation}
where $-R(t)\in N_C(x(t))$. Due to the fact that $C$ is convex, the normal cone inclusion $-R \in N_C(x)$, $x\in C$ implies $-R\T (y-x) \leq 0$ $\forall y\in C$. We denote the minimizer of \eqref{eq:fundProb} by $x^*\in C$. From the strong convexity of $f$ we obtain
\begin{align*}
f(x^*)&\geq f(y) + \left.\frac{\partial f}{\partial x}\right|_{y} (x^*-y) + \frac{\mu}{2} |x^*-y|^2
\geq f(y) + (\left.\frac{\partial f}{\partial x}\right|_{y} - R\T) (x^*-y) + \frac{\mu}{2} |x^*-y|^2,
\end{align*}
for any $y\in C$, $-R\in N_C(y)$. However, the latter inequality can be replaced with
\begin{align*}
f(x^*) \geq \min_{x\in \mathbb{R}^n} f(y) + \Big(\left.\frac{\partial f}{\partial x}\right|_{y} - R\T\Big) (x-y) + \frac{\mu}{2} |x-y|^2 = f(y) - \frac{\mu}{2} \Big| \left.\frac{\partial f}{\partial x}\right|_{y}-R\T\Big|^2,
\end{align*}
which in view of \eqref{eq:tmpproof1} yields (with $y=x(t)$)
\begin{equation*}
\frac{\diff}{\diff t}( f(x(t))-f(x^*) ) = \frac{\diff}{\diff t} f(x(t)) \leq -\frac{2}{\mu} (f(x(t)) -f(x^*)),
\end{equation*}
proving the desired convergence rate.
\end{proof}


\section{Discretization and numerical implementation}
For know the constrained gradient flow dynamics have been defined for $x(t)\in C$. In the context of optimization, however, it is often undesirable to assume that the initial condition $x(0)$ is feasible and we seek to extend the dynamics to all of $\mathbb{R}^n$. This is achieved by extending the set-valued force laws, \eqref{eq:velLevel1} and \eqref{eq:velLevel2}, to include the cases where $g_j(x(t))<0$ and $h_i(x(t))\neq 0$. We propose the following extension for the equality constraint:
\begin{equation}
\gamma_{\text{h}i}^+(\dot{x}(t),x(t)) + \alpha h_i(x(t))=0 \quad \lambda_{\text{h}i}^+(t)\in \mathbb{R}, \quad \forall t\in [0,\infty), \label{eq:condvel1}
\end{equation}
where $\alpha>0$ is constant. For $h_i(x(t))=0$ the constraint reduces to \eqref{eq:velLevel1}. However, for $h_i(x(t))\neq 0$ we obtain
\begin{equation*}
\frac{\diff}{\diff t}( h(x(t)) )^+=\gamma_{\text{h}i}^+(\dot{x}(t),x(t))=-\alpha h_i(x(t)),
\end{equation*}
which implies $h_i(x(t)) = h_i(x(0)) \exp(-\alpha t)$ for all $t\in [0,\infty)$, i.e. exponential convergence with rate $\alpha$ to the constraint manifold $h_i(x)=0$. We thus replace \eqref{eq:velLevel1} with 
\begin{equation*}
-\lambda_\text{h}^+(t) \in N_{\{0\}}\left( \gamma_\text{h}^+(\dot{x}(t),x(t))+ \alpha h(x(t))\right), \quad \forall t\in [0,\infty).
\end{equation*}
Similarly, we extend the inequality constraints to
\begin{equation}
\gamma_{\text{g}i}^+(\dot{x}(t),x(t)) + \alpha g_i(x(t))\geq 0, \quad \lambda_{\text{g}i}^+(t)\geq 0, \quad \left(\gamma_{\text{g}i}^+(\dot{x}(t),x(t)) + \alpha g_i(x(t))\right) \lambda_{\text{g}i}^+(t)=0, \label{eq:condvel2}
\end{equation}
for all $i$ such that $g_i(x(t))\leq 0$ and all $t\in [0,\infty)$. The values $\lambda_\text{gi}(t)$ are again set to zero for $g_i(x(t))>0$.  In case $g_i(x(t))$ happens to be zero we recover the original constraint \eqref{eq:velLevel2}. However, in case $g_i(x(t_0))\leq 0$ at some time $t_0\geq 0$, we obtain from 
\begin{equation*}
\gamma_{\text{g}i}^+(\dot{x}(t),x(t)) + \alpha g_i(x(t))\geq 0,\quad \forall t\geq t_0~~~\text{s.t.}~~~g_i(x(t))\leq 0,
\end{equation*}
that $g_i(x(t))\geq g_i(x(t_0)) \exp(-\alpha (t-t_0))$ for all $t\in [t_0,\infty)$, which implies that $g_i(x(t))$ likewise converges to the boundary of the manifold $g_i(x)\geq 0$. Summarizing we therefore replace \eqref{eq:velLevel2} with
\begin{equation*}
-\lambda_{\text{g}I(x)}^+ \in N_{\mathbb{R}_{\geq 0}}\left( \gamma_{\text{g}I(x)}(\dot{x},x) + \alpha g_{I(x)}(x) \right), \quad -\lambda_{\text{g}I^{\text{c}}(x)}=0,
\end{equation*}
where the dependence on time has been omitted, and where we redefine $I(x)$ as $I(x):=\{i\in \mathbb{Z}~|~g_i(x)\leq 0\}$ and its complement $I^{\text{c}}(x)$ as $I^{\text{c}}(x):=\{i\in \mathbb{Z}~|~g_i(x)>0\}$. 

%\textcolor{red}{Need to think more about this.}
In addition we extend Assumption~\ref{Ass:Fund} in the following way
\begin{assumption}\label{Ass:Fund2}
For any $x\in \mathbb{R}^n$ the rows of $\partial h/\partial x|_{x}$ are linearly independent. Moreover, there exists a vector $w\in \mathbb{R}^n$ such that $\partial h/\partial x|_{x} w=0$ and $\partial g_{I(x)}/\partial x|_{x} w > 0$.
\end{assumption}

Thus, we obtain the following generalization of \eqref{eq:tmp1},
\begin{equation}
\dot{x} + \left.\frac{\partial f}{\partial x}\right|_{x}\T = W \lambda, \quad -\lambda \in N_{D}(W\T \dot{x} + \alpha \bar{g}(x)), \label{eq:tmp2}
\end{equation}
where $\bar{g}(x):=(h(x),g_{I(x)}(x))$. In case $x(t)\in C$, \eqref{eq:tmp2} reduces to \eqref{eq:tmp1}. Similar arguments show that under Assumption~\ref{Ass:Fund2}, \eqref{eq:tmp2} the forward evolution of the trajectory $x(t)$ is unique and well-defined. In particular, \eqref{eq:tmp2} can be regarded as the following stationarity condition
\begin{equation}
\min_{\dot{x} \in \mathbb{R}^n} \frac{1}{2} \Big| \dot{x} + \left.\frac{\partial f}{\partial x}\right|_{x}\T \Big|^2 \quad \text{s.t.} \quad W\T \dot{x} + \alpha \bar{g}(x)\in D. \label{eq:Gauss2}
\end{equation}
\begin{proposition}\label{Prop:Slater}
Assumption~\ref{Ass:Fund2} implies that for all $x\in \mathbb{R}^n$, there exists a $\dot{x}\in \mathbb{R}^n$ such that $\partial h/\partial x|_{x} \dot{x} + \alpha h(x)=0$ and $\partial g_{I(x)}/\partial x|_{x} \dot{x} + \alpha g_{I(x)}(x)>0$.
\end{proposition}
\begin{proof}
We pick a $v\in \mathbb{R}^n$ such that $\partial h/\partial x|_{x}~v=-\alpha h(x)$. Due to the fact that the rows of $\partial h/\partial x|_{x}$ are linearly independent, such a $v$ exists. Thus, for a sufficiently large constant $\xi>0$, we have that $\partial h/\partial x|_{x} (v+\xi w) =-\alpha h(x)$, $\partial g_{I(x)}/\partial x|_{x} (v+ \xi w) > -\alpha g_{I(x)}(x)$, where $w\in \mathbb{R}^n$ satisfies $\partial h/\partial x|_{x} w = 0$ and $\partial g_{I(x)}/\partial x|_{x} w > 0$. The existence of such a $w$ follows from Assumption~\ref{Ass:Fund2}. Thus, $\dot{x}=(v+ \xi w)$ satisfies the required conditions.
\end{proof}
Thus, \eqref{eq:Gauss2} is a convex quadratic program, which satisfies Slater's conditions, according to Prop.~\ref{Prop:Slater}. This implies that the minimum in \eqref{eq:Gauss2} is attained, the minimizer is unique, and that for each $x\in \mathbb{R}^n$, there exists well-defined, finite dual variables $\lambda$. We now prove that the extended gradient flow according to \eqref{eq:tmp2} converges likewise to a stationary point of \eqref{eq:fundProb} and achieves the same convergence rate as stated in Prop~\ref{Prop:Conv1} on strongly convex functions, provided that $\alpha>2\mu/L$.

\begin{proposition}
Under Assumption~\ref{Ass:Fund2} and Assumption~\ref{Ass:Sol}, the constrained gradient flow as given by \eqref{eq:tmp2} has a well-defined and unique solution in forward time. The trajectory $x(t)$ necessarily converges to a stationary point of \eqref{eq:fundProb}. In case $f$ is strongly convex and smooth, the set $C$ is convex, and $\alpha>4\mu/L$, the trajectories converge with rate
\begin{equation*}
-(h(x(0)),\min\{0,g(x(0))\})\T \lambda e^{-\alpha t} \leq f(x(t))-f^*\leq (f(x(0)-f^* + c_2) e^{-2\mu t/L},
\end{equation*}
where $c_2$ is constant and $\lambda$ is any multiplier satisfying the KKT conditions of \eqref{eq:fundProb}.
\end{proposition}
\begin{proof}
For any $x(0)\in \mathbb{R}^n$ the solution $x(t)$ is well-defined according to the above reasoning. Furthermore, by construction, $x(t) \in C(t)$, where $C(t)$ is defined as
\begin{equation*}
C(t):=\{x\in \mathbb{R}^n~|~h(x)=h(x(0))\exp(-\alpha t), \quad g(x)\geq \min\{0, g(x(0))\} \exp(-\alpha t)\}.
\end{equation*}
The set $C(t)$ is closed, includes $C$ for all times $t\in [0,\infty)$, and converges to $C$ ($C(t)$ is monotonically decreasing, since $C(t_2) \subset C(t_1)$ for any $t_2\geq t_1\geq 0$).
By assumption, $x(t)$ is continuous, and since $\lim_{t \rightarrow \infty} x(t)\in C$, which is compact, it follows that $x(t)$ is bounded. As a result for each $t\in [0,\infty)$, there are bounded dual variables $\lambda(t)$ satisfying \eqref{eq:tmp2}, and in particular there exists a finite constant $c>0$ such that $\sup_{t\in [0,\infty)} |\lambda(t)|<c$. We multiply \eqref{eq:tmp2} by $\dot{x}(t)$ and rearrange terms
\begin{equation}
\diff f(x(t))/\diff t=-|\dot{x}(t)|^2 +\dot{x}(t)\T W \lambda(t). \label{eq:proofeq2}
\end{equation}
According to \eqref{eq:condvel1} and \eqref{eq:condvel2} it follows that 
\begin{equation*}
\dot{x}(t)\T W \lambda(t)=-\alpha \bar{g}(x(t))\T \lambda(t)\leq -\alpha (h(x(0)),\min\{0,g_{I(x(t))}(x(0))\})\T \lambda(t)~\exp(-\alpha t),
\end{equation*}
where $\bar{g}(x(t))$ denotes the active constraints, i.e. $\bar{g}(x(t))=(h(x(t)),g_{I(x(t))}(x(t)))$. This concludes that
\begin{align*}
f(x(t))-f(x(0)) &= \int_{0}^{t} -|\dot{x}(\tau)|^2 \diff \tau + \int_{0}^{t} -\alpha \bar{g}(x(\tau))\T \lambda(\tau) \diff \tau\\
&\leq \int_0^{t} -|\dot{x}(\tau)|^2 \diff \tau + c \int_{0}^{t} \alpha \exp(-\alpha \tau) |\bar{g}(x(0))| \diff \tau\\
&\leq \int_{0}^{t} - |\dot{x}(\tau)|^2 \diff \tau + c |\bar{g}(x(0))|.
\end{align*}
Moreover, since $f(x(t))-f(x(0))$ is bounded below ($f(x(t))$ is continuous in $t$ and $\lim_{t\rightarrow \infty} f(x(t))$ is bounded below, since $\lim_{t\rightarrow \infty} x(t)\in C$) it follows that the above right-hand side converges, which implies that $\lim_{t\rightarrow \infty} \dot{x}^+(t) \rightarrow 0$. Thus, $x(t)$ converges to a point in $C$ for $t\rightarrow \infty$ (by continuity of $g$ and $h$) and $\lim_{t\rightarrow \infty} x(t)$ satisfies \eqref{eq:KKT} and is therefore a stationary point of \eqref{eq:fundProb}. In case $f$ is strongly convex and smooth, and $C$ is convex, we obtain from the same reasoning as in Proposition~\ref{Prop:ConvGD} that 
\begin{equation*}
-|\dot{x}(t)|^2 = -\Big|-\left.\frac{\partial f}{\partial x}\right|_{x(t)} +R(t)\Big|^2 \leq -\frac{2}{\mu} (f(x(t))-f(x^*)).
\end{equation*}
In view of \eqref{eq:proofeq2} we therefore obtain
\begin{equation*}
\frac{\diff}{\diff t}(f(x(t))-f(x^*))\leq -\frac{2}{\mu} (f(x(t))-f(x^*)) + c \alpha \exp(-\alpha t) |\bar{g}(x(0))|,\quad \forall t\in [0,\infty),
\end{equation*}
implying that
\begin{equation*}
f(x(t))-f(x^*)\leq \exp(-2 t/\mu) \left( f(x(0))-f(x^*) + c \alpha |\bar{g}(x(0))| \int_{0}^{t} \exp((2/\mu - \alpha) \tau)\diff \tau\right).
\end{equation*}
Thus, for $\alpha>2/\mu$, the integral on the right-hand side remains bounded for $t\rightarrow \infty$, which leads to the desired upper bound.

The lower bound follows from a perturbation analysis. We define $f^*(t):=\inf_{x\in C(t)} f(x)$, which is of the form \eqref{eq:fundProb}, with the sole difference that the right-hand-side of the constraints has been replaced with the vector $v \exp(-\alpha t)$, where $v:=(h(x(0)),\min\{0,g(x(0))\})$. A multiplier $\lambda$ satisfying the KKT conditions of \eqref{eq:fundProb} is quaranteed to satisfy (see \cite[p.~277]{RockafellarConvex})
\begin{equation*}
f^*(t)-f^*\geq -\lambda\T v \exp(-\alpha t),
\end{equation*}
where $\lambda\T v>0$ (as can be seen, for example, from $\lim_{t\rightarrow \infty} f^*(t)=f^*$). The lower bound then follows from the fact that $f(x(t))\geq f^*(t)$ for all $t\in [0,\infty)$.
\end{proof}



There are many different possibilities to discretize the constrained gradient flow dynamics given by \eqref{eq:tmp2}. We focus on the forward Euler scheme, whereby we replace the velocity $\dot{x}(t)$ (or $\dot{x}(t)^+$) by the finite difference $(x_{k+1}-x_{k})/T$, where $T>0$ is a fixed time step. This amounts to 
\begin{equation*}
x_{k+1}=x_{k} -T \left.\frac{\partial f}{\partial x}\right|_{x_k}\T + T W_k \lambda_k, \quad W_k:=\left( \left.\frac{\partial h}{\partial x}\right|_{x_k}\T, \left.\frac{\partial g_{I(x_k)}}{\partial x}\right|_{x_k}\T \right),
\end{equation*}
where $-\lambda_k \in N_{D}(W_k\T (x_{k+1}-x_{k})/T + \alpha \bar{g}(x_k))$. In order to calculate the magnitude of the constraint forces $\lambda_k$ we reformulate the normal cone inclusion for $\lambda_k$ using the dual cone $D^*$, which yields (similar to \eqref{eq:dualProb})
\begin{equation}
W_k\T W_k \lambda_k - W_k\T \left.\frac{\partial f}{\partial x}\right|_{x_k}\T + \alpha \bar{g}(x_k) \in N_{D^*}(-\lambda_k). \label{eq:ncInclfinal}
\end{equation}
A normal cone inclusion can be further rewritten in terms of the proximal point operator, as is shown by the following lemma
\begin{lemma}
Let $K\subset \mathbb{R}^m$ be a closed, convex cone. Then $y\in N_K(x)$ is and only if $x=\text{prox}_K(x+Ry)$, for an arbitrary $R=\diag(r_1,\dots,r_m)>0$.
\end{lemma}
As a consequence, \eqref{eq:ncInclfinal} can be expressed as
\begin{equation}
-\lambda_k = \prox_{D^*} \Big( -\lambda_k + R \Big(W_k\T W_k \lambda_k - W_k\T \left.\frac{\partial f}{\partial x}\right|_{x_k}\T + \alpha \bar{g}(x_k) \Big)\Big),
\end{equation}
which can be efficiently solved by fixed-point iteration. It is important to note that the $\text{prox}_{D^*}$ is computationally cheap to evaluate, since $D^*:=\{0\}^{n_\text{h}} \times \mathbb{R}_{\leq 0}^{|I(x)|}$. Compared to projected gradient descent, we therefore only perform projections on the dual variables $\lambda_k$. 
\newpage

We recall that $-\lambda \in N_D(x)$ if and only if $-\lambda\T \delta x \leq 0$ for all $\delta x\in T_D(x)$, or equivalently if and only if $-\lambda \in \partial \psi_D(x)$, where $\partial \psi_D$ denotes the subdifferential of the indicator function $\psi_D$ of the convex set $D$. As a result, \eqref{eq:tmp1} can be interpreted as as stationarity condition of a corresponding convex quadratic problem
\begin{equation}
-\dot{x}-\left.\frac{\partial f}{\partial x}\right|_{x}\T \in W \partial \psi_D(W\T \dot{x})\quad \Leftrightarrow \quad \min_{\dot{x} \in \mathbb{R}^n} |\dot{x} + \left.\frac{\partial f}{\partial x}\right|_{x}\T |^2, \quad \text{s.t.} \quad W\T \dot{x} \in D.
\end{equation}


due to the assumption that $\dot{x}$ is of locally bounded variation. Combined with the set-valued force laws this implicitly describes the velocity $\dot{x}^+(t)$ 

For obtaining an efficient optimization algorithm, it is useful to express the conditions \eqref{eq:posLevel} in terms of the rate of change of an absolutely continuous trajectory $x(t)$, assuming that $x(t)\in C$. Transforming the equality constraints is straight-forward. Provided that $h(x(t))=0$ for some time instant $t$, $h(x(t))$ will remain zero if and only if $\partial h/\partial x|_{x(t)} \dot{x}(t)=0$. Hence the first condition in \eqref{eq:posLevel} can be likewise expressed as 

Condition \eqref{eq:cond2} (or equivalently \eqref{eq:cond1}) defines an optimization algorithm for \eqref{eq:fundProb}, as $\mathcal{N}_C(x)$ is guaranteed to be non-empty for any $x\in C$. 
define an optimization algorithm for \eqref{eq:fundProb}. The function $f$ necessarily decreases along a trajectory $x(t)$ that satisfies \eqref{eq:cond1}.
We tacitly assume that a trajectory $x(t)$ exists. 

From a mechanical perspective, \eqref{eq:varForm} amounts to the principle of virtual work, a fundamental postulate of classical mechanics. We restrict ourselves to mechanical systems with perfect bilateral and unilateral constraints, which are defined below. The distinction between external and internal forces is essential. 
\begin{postulate}
A mechanical system is in static equilibrium if and only if the virtual work vanishes for any virtual displacement $\delta x$. The virtual work is defined as $(F+R)\T \delta x$, where $F$ is the sum of all external forces and $R$ is the sum of all constraint forces.
\end{postulate}\label{Pos:VirtWork}
In that sense, $-\partial f/\partial x\T$ amounts to the sum of external forces $F$, whereas the constraint forces $R$ are given by $\partial h/\partial x\T \lambda_\text{h} + \partial g/\partial x\T \lambda_\text{g}$. In general, constraint forces $R$ are forces that satisfy $R\T \delta x \leq 0$ for all variations $\delta x$ that are in accordance with the constraint, that is $\delta x \in T_C(x^*)$.
This leads to the following corollary of the principle of virtual work, commonly referred to the principle of D'Alembert-Lagrange
\begin{corollary}
If a mechanical system is in static equilibrium, the virtual work of the external forces satisfies $F\T \delta x \leq 0$ for all $\delta x$ that are admissible, i.e. $\delta x \in T_C(x^*)$.
\end{corollary}

From a mechanical perspective, \eqref{eq:statCond} and \eqref{eq:KKT} are different formulations of the principle of virtual work and the principle of d'Alembert-Lagrange. The principle of virtual work states that the mechanical system is in static equilibrium if and only if the virtual work $\delta \bar{W}$ satisfies $\delta \bar{W} \leq 0$ for all admissible variations.

To obtain \eqref{eq:KKT} from \eqref{eq:statCond}, we essentially replaced each constraint encoded with $\delta x\in T_C(x^*)$, by a corresponding constraint force, which is required to be normal to $T_C(x^*)$ in the sense that
\begin{equation*}
\left(-\lambda_\text{h}\T \left.\frac{\partial h}{\partial x}\right|_{x^*} - \lambda_\text{g}\T \left.\frac{\partial g}{\partial x}\right|_{x^*} \right) \delta x \leq 0, \quad \forall \delta x \in T_C(x^*).
\end{equation*}
 The situation is illustrated on a few examples in Fig.~\ref{Fig:illustration}.

